Hierarchical Control for Vehicle Repositioning in Autonomous Mobility on Demand Systems

Balancing passenger demand and vehicle availability is crucial for ensuring the sustainability and effectiveness of urban transportation systems. To address this challenge, we propose a novel hierarchical strategy for the efficient distribution of empty vehicles in urban areas. The proposed approach employs a data-enabled predictive control algorithm to develop a high-level controller, which guides the inter-regional allocation of idle vehicles. This algorithm utilizes historical data on passenger demand and vehicle supply in each region to construct a non-parametric representation of the system, enabling it to determine the optimal number of vehicles to be repositioned or retained in their current regions without modeling the system. At the low level, a coverage control-based controller is designed to provide inter-regional position guidance, determining the desired road intersection each vehicle should target. With the objective of optimizing area coverage, it aligns the vehicle distribution with the demand across different districts within a single region. The effectiveness of the proposed method is validated through simulation experiments on the real road network of Shenzhen, China. The integration of the two layers provides better performance compared to applying either layer in isolation, demonstrating its potential to reduce passenger waiting time and answer more requests, thus promoting the development of more efficient and sustainable transportation systems.

==> section/Preliminary.tex <==
\subsection{Preliminary}\label{subsec: preliminary}
\section{Review of Data-enabled Predictive Control}\label{Preliminary}
In this section, we recall the main result of \cite{WILLEMS2005} on non-parametric system representation, and then we give a brief review of the DeePC algorithm proposed in \cite{Coulson2018}.
\subsection{Preliminaries}
Consider a discrete-time Linear Time-Invariant (LTI) system as
% %\begin{linenomath}
\begin{equation}
\Bigl\{
    \begin{array}{cc}
       x_{k + 1}&=Ax_k+Bu_k\\
       y_k &=Cx_k+Du_k,
       \end{array}\label{LTI}
       \end{equation}
% %\end{linenomath}
where $x_k \in \mathbb{R}^{n}$ is the state vector, $u_k \in \mathbb{R}^{m}$ is the control input vector, and $y_k \in \mathbb{R}^p$ is the output vector of the system at time $k \in \mathbb{Z}$. $ A \in \mathbb{R}^{n \times n}$, $B\in \mathbb{R}^{n \times m}$, $C\in \mathbb{R}^{p \times n}$, and $D\in \mathbb{R}^{p \times m}$. Instead of learning $A, B, C$ and $D$ via system identification to obtain a parametric representation of the system, we are interested in the case when $A, B, C$ and $D$ are unknown but the input and output data samples, i.e., $u = col(u_1, u_2,\dots)$ and $y = col(y_1,y_2,\dots)$ are available.
Note here $col(a_1,a_2,\dots,a_i) := [a_1^T;a_2^T;\dots;a_i^T]^T$.



\textbf{\textit{Theorem 1 (\cite{WILLEMS2005})}}. Let $L,T_d\in \mathbb{Z}$. Collected from unknown system (\ref{LTI}), $u^d = col(u_1,u_2,\dots,u_{T_d})$ and $y^d = col(y_1, y_2, \dots,y_{T_d})$ are input and output trajectory of length $T_d$, such that $u^d$ is persistently exciting of order $L + n$. Then $(u, y)$ is a trajectory of system (\ref{LTI}) if and only if there exists $g\in \mathbb{R}^{T_d-L+1}$ such that
%\begin{linenomath}
\begin{equation}\left[
    \begin{array}{cc}
         \mathcal{H}_L(u^d)\\
        \mathcal{H}_L(y^d)
    \end{array}\right] g = 
\left[
    \begin{array}{cc}

         u\\
         y
    \end{array}\right].\label{Hankel_theorem}
\end{equation}

Theorem 1 indicates that the subspace spanned by the columns of Hankel matrix $\left[\begin{smallmatrix}
\mathcal{H}_L(u^d)\\
        \mathcal{H}_L(y^d)
\end{smallmatrix}\right]$ corresponds to the subspace of all possible trajectories of the system (\ref{LTI}).

Furthermore, let $T_{ini}, N\in\mathbb{Z}$ be the lengths of time horizon for initial condition estimation and future prediction, respectively. The Hankel matrices constructed by $u^d$ and $y^d$ are partitioned into two parts, where the superscript `$p$' stands for `past data' and `$f$' for `future data' as
\begin{equation}\label{hankel_u}\left[
    \begin{array}{cc}
           U^p\\
          U^f
    \end{array}\right]:=\mathcal{H}_{T_{ini}+N}(u^d), 
\end{equation}
\begin{equation}\label{hankel_y}\left[
    \begin{array}{cc}
           Y^p\\
          Y^f
    \end{array}\right]:=\mathcal{H}_{T_{ini}+N}(y^d),
\end{equation}
where $U^p\in \mathbb{R}^{mT_{ini}\times(T_d-T_{ini}-N+1)}$ consists of the first $mT_{ini}$ block row of $\mathcal{H}_{T_{ini}+N}(u^d)$ , and $U^f\in \mathbb{R}^{mN\times(T_d-T_{ini}-N+1)}$ consists of the last $mN$ block row of $\mathcal{H}_{T_{ini}+N}(u^d)$. Similarly, $Y^p\in \mathbb{R}^{pT_{ini}\times(T_d-T_{ini}-N+1)}, Y^f\in \mathbb{R}^{pN\times(T_d-T_{ini}-N+1)}$.

According to \cite{Huang2022}, compared to system (\ref{LTI}), a measurable external disturbance is considered additionally and this unknown LTI system can be expressed as 
\begin{equation}
\Bigl\{
    \begin{array}{cc}
       x_{k + 1}&=Ax_k+Bu_k + B_d w_k\\
       y_k &=Cx_k+Du_k + D_d w_k,
       \end{array}\label{LTI_dist}
       \end{equation}
where $w_k \in \mathbb{R}^q$ is the disturbance variable, and $B_d \in \mathbb{R}^{n \times q}$ and $D_d \in \mathbb{R}^{p \times q}$. 
% Assume that we are able to measure the historical trajectory of length $T_d$  the external disturbance $w^d$ as well as $(u^d, y^d)$, however the future is unknown. \in \mathbb{R}^{qT_d} 

Considering $w_k$ as an uncontrollable input, similar to \cref{hankel_u} and \cref{hankel_y}, we can construct another Hankel matrix regarding the disturbance and further partition it into two parts as
\begin{equation}\label{hankel_w}\left[
    \begin{array}{cc}
           W^p\\
          W^f
    \end{array}\right]:=\mathcal{H}_{T_{ini}+N}(w^d), 
\end{equation}
where $W^p\in \mathbb{R}^{qT_{ini}\times(T_d-T_{ini}-N+1)}, W^f\in \mathbb{R}^{qN\times(T_d-T_{ini}-N+1)}$. Assume that a historical trajectory of external disturbance $w^d$ of length $T_d$ is measured such that $col(u^d, w^d)$ is persistently exciting of order $T_{ini} + N + n$ \cite{Huang2022}. According to 
\textit{Theorem 1}, $col(u,w,y)$ is a possible future trajectory of system (\ref{LTI_dist}) of initial condition $col(u_{ini}, w_{ini}, y_{ini})$, if and only if there exist  $g\in R^{T_d-T{ini}-N+1}$ such that 
%\begin{linenomath}
\begin{equation}\left[
    \begin{array}{cccc}
         U^p\\
         W^p\\
         Y^p\\
         U^f\\
         W^f\\
         Y^f\\
    \end{array}\right] g = 
\left[
    \begin{array}{cccc}
         u_{ini}\\
         w_{ini}\\
         y_{ini}\\
         u\\
         w\\
         y\\
    \end{array}\right].\label{Hankel_uwy}
\end{equation}


% Suppose $u^d$ is persistently exciting of order $T_{ini} + N + n$, and $col(u_{ini},y_{ini})$ is the most recent input and output measurements from this system. According to \cref{Hankel_theorem}, $col(u,y)$ is a possible future trajectory of system (\ref{LTI}) if and only if there exist $g\in R^{T-T{ini}-N+1}$ such that 
% %\begin{linenomath}
% \begin{equation}\left[
%     \begin{array}{cccc}
%          U^p\\
%          Y^p\\
%          U^f\\
%          Y^f\\
%     \end{array}\right] g = 
% \left[
%     \begin{array}{cccc}
%          u_{ini}\\
%          y_{ini}\\
%          u\\
%          y\\
%     \end{array}\right].\label{Hankel_uy}
% \end{equation}

% In other words, $col(u_{ini}, w_{ini}, y_{ini}, u, w, y)$ can be seen as a trajectory that starts with the initial condition $col(u_{ini}, w_{ini}, y_{ini})$ and a future trajectory $col(u, w,  y)$ departing from this initial condition \cite{Coulson2018}. 
Therefore, the Hankel matrix constructed directly by raw data can serve as a non-parametric model representing the system behavior, bypassing the parameter identification of the system model. Next, we will implement optimal predictive control with the constructed Hankel matrices.


\subsection{Review of Data-enabled Predictive Control (DeePC)}
% Let $T_{ini}, N\in\mathbb{Z}$  The input and output trajectory which are collected from this unknown system are $u^d\in\mathbb{R}^{mT}$ and $y^d\in\mathbb{R}^{pT}$ respectively,  The Hankel matrices can be constructed by $u^d$ and $y^d$, and are further partitioned into two parts as

%\end{linenomath}
%\begin{linenomath}
% \begin{equation}\left[
%     \begin{array}{cccc}
%          U^p\\
%          Y^p\\
%          \textcolor{red}{E^P}\\
%          U^f\\
%          Y^f\\
%          \textcolor{red}{E^f}
%     \end{array}\right] g = 
% \left[
%     \begin{array}{cccc}
%          u_{ini}\\
%          y_{ini}\\
%          \textcolor{red}{e_{ini}}\\
%          u\\
%          y\\
%          \textcolor{red}{e}
%     \end{array}\right].
% \end{equation}
%\end{linenomath}
% %\begin{linenomath}
% \begin{equation}\label{deepc}
%     \begin{array}{cc}
%          \min_{g,u,y,\sigma_y} \sum_{k=0}^{N-1}(\Vert y_k - r_{t+k}\Vert^2_Q + \Vert u_k \Vert^2_R) + \lambda_g \Vert g\Vert_I ^2 + \lambda_y \Vert \sigma_y \Vert_I^2\\
%          subject \quad to \left[
%     \begin{array}{cccc}
%          U^p\\
%          Y^p\\
%          U^f\\
%          Y^f\\
%     \end{array}\right] g = 
% \left[
%     \begin{array}{cccc}
%          u_{ini}\\
%          y_{ini}\\
%          u\\
%          y\\
%     \end{array}\right] + 
%     \left[
%     \begin{array}{cccc}
%          0\\
%          \sigma_y\\
%          0\\
%          0\\
%     \end{array}\right],\\
%     u_k\in \mathcal{U},\forall k \in{0,1,\dots,N-1},\\
%     y_k\in \mathcal{Y}, \forall k \in{0,1,\dots,N-1}.\\
          
%     \end{array}
% \end{equation}
%\end{linenomath}

Viewing the collected data $col(u^d, w^d, y^d)$, the Hankel matrices can replace the system model to predict the future trajectory. DeePC \cite{Coulson2018} solves an optimization problem in a receding horizon manner, attempting to obtain optimal control actions meanwhile satisfying the input and output constraints. Considering the time horizon $N \in \mathbb{Z}$, we formulate the optimization problem as follows
% Viewing the collected data samples $col(u_{ini},y_{ini})$, DeePC learns the system's behaviour and attempts to obtain optimal control inputs meanwhile meeting the input and output constraints. Consider the time horizon $N\in Z$, a desired reference trajectory as $r = (r_0,r_1,\dots)$, where $r_i\in R^p$. We formulate the optimization problem as follows

\begin{equation}\label{deepc}
    \begin{array}{cc}
        %  \displaystyle{\min_{g,u,y,\sigma_y} \sum_{k=0}^{N-1}(\Vert y_k - r_{t+k}\Vert^2_Q + \Vert u_k \Vert^2_R) + \lambda_g \Vert g\Vert_I ^2 + \lambda_y \Vert \sigma_y \Vert_I^2}\\
        %  subject \quad to \left[
                 \displaystyle{\min_{g,u,y,\sigma_y} f(u_{k + i},y_{k + i}) + \lambda_g \Vert g\Vert_2 ^2 + \lambda_y \Vert \sigma_y \Vert_2^2}\\
         subject \quad to \left[

%    
 \begin{array}{cccc}
         U^p\\
         W^p\\
         Y^p\\
         U^f\\
         W^f\\
         Y^f\\

    \end{array}\right] g = 
\left[
    \begin{array}{cccc}
         u_{ini}\\
         w_{ini}\\
         y_{ini}\\
         u\\
         w\\
         y\\
    \end{array}\right]+ 
    \left[
    \begin{array}{cccc}
         0\\
         0\\
         \sigma_y\\
         0\\
         0\\
         0\\
    \end{array}\right],\\

    u_{k + i}\in \mathcal{U},\forall i \in{0,1,\dots,N-1},\\
    y_{k + i}\in \mathcal{Y}, \forall i \in{0,1,\dots,N-1},
    \end{array}
\end{equation}
where $f(u_{k + i},y_{k + i})$ is the control objective function. The input constraint is $\mathcal{U}\subseteq \mathbb{R}^{mN}$, output constraint is $\mathcal{Y}\subseteq \mathbb{R}^{pN}$.
% the control cost matrix is $R \in \mathbb{R}^{mN \times mN}$, and the output cost matrix is $Q \in \mathbb{R}^{pN \times pN}$.
$\Vert \cdot \Vert_{\alpha}$ denotes $\alpha$ norm. $\lambda_g \in \mathbb{R}_{>0}$ is introduced as regularization parameter to avoid data overfitting. Compared to \cref{Hankel_uwy}, $\sigma_y \in \mathbb{R}^{T_{ini}p}$ is added to the right side as an auxiliary slack variable, and a weight coefficient $\lambda_y \in \mathbb{R}_{>0}$is incorporated as well to ensure the feasibility of the constraints over all time \cite{Coulson2018}. More discussion on robust DeePC can be found in \cite{Coulson2019}.

$col(u_{ini}, w_{ini}, y_{ini})$ represents the most recent input, disturbance and output measurement and is used as the initial condition to predict the future, thus it should be updated at each time step $k$. Note that $u$ and $y$ is not independent with $g$ since by \cref{Hankel_uwy}, $u = U^fg$ and $y = Y^fg$. Solving \cref{deepc} gives an optimal control action sequence $u^* = col(u^*_k, u^*_{k+1}, \dots, u^*_{k + N - 1})$, and we only apply the first control input, i.e., $u^*_k$. 



